BenchBot: Evaluating Robotics Research in Photorealistic 3D Simulation and on Real Robots

We introduce BenchBot, a novel software suite for benchmarking the performance of robotics research across both photorealistic 3D simulations and real robot platforms. BenchBot provides a simple interface to the sensorimotor capabilities of a robot when solving robotics research problems; an interface that is consistent regardless of whether the target platform is simulated or a real robot. In this paper we outline the BenchBot system architecture, and explore the parallels between its user-centric design and an ideal research development process devoid of tangential robot engineering challenges. The paper describes the research benefits of using the BenchBot system, including: enhanced capacity to focus solely on research problems, direct quantitative feedback to inform research development, tools for deriving comprehensive performance characteristics, and submission formats which promote sharability and repeatability of research outcomes. BenchBot is publicly available (http://benchbot.org), and we encourage its use in the research community for comprehensively evaluating the simulated and real world performance of novel robotic algorithms.

==> text/case_study.tex <==
\section{Semantic scene understanding: a BenchBot case study}
\label{sec:study}

\ben{Lead in describing the scope for the ``BenchBot case study'', and what we were trying to achieve. Make sure that we mention the case study is powering the semantic scene understanding challenge.}

\subsection{Defining tasks}

\ben{Here we go from the semantic scene understanding research problem, to our two tasks (semantic SLAM and scene change detection). We need to clearly define what they are, and what parts of the research problem they attempt to address.}

\ben{Finish / make sure by the end that ``what performance is'' in these tasks has been defined. We should have the concept of a ground-truth object-based semantic map, and how it differs for scene change detection (show in Figure \ref{fig:tasks})}.

\begin{figure}[t]
  \centering
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/task_sslam.png}
    \caption{}
    \label{subfig:task_sslam}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/task_scd.png}
    \caption{}
    \label{subfig:task_scd}
  \end{subfigure}

  \caption{The object-based semantic maps used to represent results for each of the semantic scene understanding tasks: \subref{subfig:task_sslam}) semantic SLAM, and \subref{subfig:task_scd}) scene change detection (\ben{These images probably need a little tidying up in terms of consistency / visibility})}%
  \label{fig:tasks}
\end{figure}

\subsection{OMQ: a metric for semantic scene understanding}

\ben{
  Description of OMQ. Want to cover the following points, but not set on what order will work best:
  \begin{itemize}
    \item what: OMQ is a probabilistic object-based semantic map comparison, that is based on existing work in PrOD
    \item why: we can't just compare the two maps using a standard approach (IOU, etc.) because\ldots
    \item how: OMQ produces a summary score based on the quality of of each requested per-object metric in an object-based semantic map. Per-object metrics are label, position, and change state (only for scene change detection). OMQ provides ``probabilistic evaluation'' for probabilistic per-object metrics. Mention that OMQ isn't fully probabilistic as we still use IOU underneath for position of the object?
  \end{itemize}
}

\subsection{Using BenchBot to gather results}

\ben{
  These results can have any of a number of scopes. I think the best option is to pick the scope that we believe warrants RAL publication, and go no further as it gives Suman's paper more space to establish itself. My suggestions on possible results, in order of weak to strong are:
  \begin{enumerate}
    \item pretty much the tutorial showing we get a score
    \item Votenet (i.e. tutorial) across each environment (i.e. we perform semantic SLAM evaluation of the Votenet-powered system for them)
    \item same as above, but also for scene change detection
    \item same as above, but gain some rudimentary insights to help justify our tool's value to the community with some basic parameters sweeps (parameters like detection amalgamation methods, combination thresholds, and detection thresholds through Votenet)---Michael got me to do this for our IROS OpenSeqSLAM2 paper which seemed to work well with reviewers
    \item use a couple of different detectors and compare their OMQ scores to present some relative insight
    \item same as above, but semantic SLAM systems rather than just detectors
    \item comprehensively compare multiple state of the art semantic SLAM systems, do some parameter sweeps, and present significant insights into performance breakdown that are of value to the research community (definitely overkill / too far for here\ldots that's going to be Suman's paper!)
  \end{enumerate}
  My thoughts are \#3 will probably get us by, but \#4 could potentially be needed to get us across the line with RAL?
}

\ben{
  This section in the ``planting the flag'' version can be nothing more than a paragraph summarising the tutorial. The rest of the paper is solely writing up existing work, this bit is the only potential new work.
}




==> text/results.tex <==
\section{Semantic scene understanding results}
\label{sec:results}

Some examples showing what you can do with BenchBot.

